Adaptive Principal Component Regression with Applications to Panel Data

Principal component regression (PCR) is a popular technique for fixed-design error-in-variables regression, a generalization of the linear regression setting in which the observed covariates are corrupted with random noise. We provide the first time-uniform finite sample guarantees for (regularized) PCR whenever data is collected adaptively. Since the proof techniques for analyzing PCR in the fixed design setting do not readily extend to the online setting, our results rely on adapting tools from modern martingale concentration to the error-in-variables setting. We demonstrate the usefulness of our bounds by applying them to the domain of panel data, a ubiquitous setting in econometrics and statistics. As our first application, we provide a framework for experiment design in panel data settings when interventions are assigned adaptively. Our framework may be thought of as a generalization of the synthetic control and synthetic interventions frameworks, where data is collected via an adaptive intervention assignment policy. Our second application is a procedure for learning such an intervention assignment policy in a setting where units arrive sequentially to be treated. In addition to providing theoretical performance guarantees (as measured by regret), we show that our method empirically outperforms a baseline which does not leverage error-in-variables regression.

==> arxiv/external_technical_lemmas.tex <==
\section{External Technical Lemmas}

In this section, we state several technical Lemmas that are needed for constructing the confidence sets and performing the regret analysis in this work.

\begin{lemma}[\textbf{Method of Mixtures}]
\label{lem:ext:mixture}
Let $(\calF_t)_{t \geq 0}$ be a filtration. Let $S_t = \sum_{s = 1}^t \epsilon_s X_s$ where $(\epsilon_t)_{t \geq 1}$ is an $(\calF_t)_{t \geq 0}$-adapted $\R$-valued $\sigma$-subGaussian random variables and $(X_t)_{t \geq 1}$ is an $(\calF_t)_{t \geq 1}$-predictable $\R^d$-valued process. Let $\rho > 0$ be arbitrary, and let 
$$
\cV_t := \sum_{s = 1}^t X_s X_s^T + \rho I_d.
$$
Let $\delta \in (0, 1)$ be any confidence parameter. Then, we have, with probability at least $1 - \delta$, simultaneously for all $t \geq 1$,
$$
\left\|V_t^{-1/2}S_t\right\|_2 \leq \sigma\sqrt{2\log\left(\frac{1}{\delta}\sqrt{\det(\rho^{-1}\cV_t)}\right)}.
$$
\end{lemma}
\begin{comment}
\begin{lemma}[\textbf{Hanson-Wright Inequality}]
\label{lem:ext:hanson}
Let $\zeta \in \R^{t}$ be a random vector such that $\zeta_s$ is $\sigma$-subGaussian for each $s \in [t]$, and let $\vA \in \R^{t \times t}$ be a fixed matrix. Then, there is a universal constant $C > 0$ such that, for any $t > 0$,
$$
\P\left(\zeta^T\vA\zeta - \E\left[\zeta^T \vA \zeta\right] \geq t\right) \leq \exp\left\{-C\min\left\{\frac{-t^2}{\sigma^4\|\vA\|_F^2}, \frac{-t}{\sigma^2\|\vA\|_{op}}\right\}\right\}
$$
\end{lemma}
\end{comment}

\begin{lemma}[\textbf{Weyl's Inequality}]
\label{lem:ext:weyl}
Let $\vA, \vB \in \R^{t \times n}$. Then, for any $i \in [t \land n]$, we have
$$
\left|\sigma_i(\vA) - \sigma_i(\vB)\right| \leq \left\|\vA - \vB\right\|_{op}.
$$


\end{lemma}

\begin{lemma}[\textbf{Wedin's Lemma}]
\label{lem:ext:wedin}
Let $\vA, \vB \in \R^{t \times n}$, and suppose $\vA$ and $\vB$ have spectral decompositions 
$$
\vA = \vU \Sigma \vV^T \qquad \text{and} \qquad \vB = \wh{\vU} \wh{\Sigma} \wh{\vV}^T.
$$
Then, for any $r$, we have 
$$
\max\left\{\left\|\vU_r\vU_r^T - \wh{\vU}_r\wh{\vU}_r^T\right\|_{op}, \left\|\vV_r\vV_r^T - \wh{\vV}_r\wh{\vV}_r^T\right\|_{op}\right\} \leq \frac{2\left\|\vA - \vB\right\|_{op}}{\sigma_r - \sigma_{r + 1}}.
$$
\end{lemma}

\begin{lemma}
\label{lem:ext:noise_bound}
Let $W \subset \R^d$ be a fixed subspace with $\dim(W) = r$. Let $\epsilon_1, \dots, \epsilon_t \in W$ be a sequence of independent, mean zero random vectors such that $\|\epsilon_i\|_{\psi_2} \leq K$, for all $i \in [t]$. Then, letting $\Epsilon_t := (\epsilon_1, \dots, \epsilon_t)^T$, there are absolute constants $C_1, C_2 > 0$1 such that, with probability at least $1 - \delta$, we have
\begin{align*}
\left\|\Epsilon_t^T\Epsilon_t - \E\left[\Epsilon_t^T\Epsilon_t\right]\right\|_{op} &\leq K^2\left(C_1\sqrt{r} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)\max\left\{\sqrt{t}, C_1\sqrt{r} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right\} \\
&\leq K^2C_2\left(\sqrt{r} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)\left\{\sqrt{t} + \sqrt{r} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right\} 
\end{align*}

    
\end{lemma}

\begin{lemma}
\label{lem:ext:noise_cov}
Let $\epsilon_1, \dots, \epsilon_t \in \R^d$ be a sequence of independent, mean zero random vectors such that $\|\E[\epsilon_i\epsilon_i^T]\|_2 \leq \gamma$, for all $i \in [t]$. Then, letting $\Epsilon_t := (\epsilon_1, \dots, \epsilon_t)^T$, we have

$$
\left\|\E\left[\Epsilon_t^T\Epsilon_t\right]\right\|_{op} \leq t\gamma.
$$
    
\end{lemma}

\begin{lemma}[\textbf{Determinant-Trace Inequality}]
\label{lem:ext:det_trace}
Let $\vA \in \R^{d \times d}$ be a positive-semidefinite matrix of rank $r$. Then, for any $\rho > 0$, we have
$$
\log\det(I_d + \rho^{-1}A) \leq r\log\left(1 + \frac{\sigma_1(\vA)}{\rho}\right).
$$

\end{lemma}

\begin{proof}
We have
\begin{align*}
\log\det(I_d + \rho^{-1}(\vA)) &= r\log\left[\det(I_d + \rho^{-1}(\vA))^{1/r}\right] \\
& = r\log\prod_{i = 1}^r\left(1 + \rho^{-1}\sigma_i(\vA)\right)^{1/r} \\
&\leq r\log\left(\sum_{i = 1}^r\frac{1 + \rho^{-1}\sigma_i(\vA)}{r}\right) \\
&\leq r\log\left(1 + \frac{\sigma_1(\vA)}{\rho}\right).
\end{align*}

\end{proof}

The following unites traditional characterizations of sub-Gaussianity with those involving Orlicz norms. See \citet{vershynin2018high} for additional details.

\begin{lemma}[\textbf{Equivalent Characterizations of SubGaussianity}]
\label{lem:ext:subg}
Suppose $X$ is a random variable that is $\sigma$-subGaussian, i.e. $\log\E e^{\lambda X} \leq e^{\lambda^2\sigma^2/2}$ for all $\lambda \in \R$. Then, there is some universal constant $C_1 > 0$ such that $\|X\|_{\psi_2} \leq C_1 \sigma$. Likewise, suppose $Y$ is mean zero and that $\|Y\|_{\psi_2} \leq K$. Then, there some other universal constant $C_2 > 0$ such that $Y$ is $C_2 K$-subGaussian.

\end{lemma}

An important mathematical object in our analyses will the be the \textbf{$(d, k)$-Grassmannian manifold}, which is the manifold $G_{d, k}$ defined as
$$
G_{d, k} := \left\{ E \subset \R^d : E \text{ is a linear subspace},\; \dim(E) = k\right\}.
$$
There are a variety of metrics that can be applied to $G_{d, k}$, but for our applications a metric of particular interest is $d_\infty : G_{d, k} \times G_{d, k} \rightarrow \R_{\geq 0}$ given by
$$
d_\infty(E, F) := \left\|\vP^E - \vP^F\right\|_{op},
$$
where we recall $\vP^W$ is the projection operator onto the linear subspace $W$. In particular, the covering number of $G_{d, k}$ will prove useful.

\begin{lemma}[\textbf{Proposition 8 in \citet{pajor1998metric}}]
There is a constant $C > 0$ such that, for any $1 \leq k \leq d$ and $\epsilon > 0$, we have
$$
N(G_{d, k}, d_\infty, \epsilon) \leq \left(\frac{C}{\epsilon}\right)^{k(d - k)}.
$$


\end{lemma}

==> arxiv/general_problem.tex <==
\section{Bandits with Noisy Contexts}
\subsection{Problem Setup}

We describe the general ``contextual bandits with noisy contexts'' problem in this subsection. An agent sequentially interacts with an environment over a sequence of rounds $t \in \{1, \dots, T\}$ for some pre-fixed time horizon $T$. At the start of each round, the environment generates some context $X_t \in W^\ast \subset \R^d$, where $W^\ast$ is a lower-dimensional linear subspace of dimension $\dim(W^\ast) = r$. We assume $r$ is known to the learner. The environment then releases a noisy version of the context given by $Z_t := X_t + \epsilon_t$ to the agent.

Given such a noisy context $Z_t$, the agent then selects an action $a_t \in \{1, \dots, A\}$, and then receives reward $Y_t := \langle \theta(a_t), X_t \rangle + \xi_t$, where $\xi_t$ is another noise variable, and $\theta(a)$ for $a \in [A]$ are unknown slope vectors lying in $W^\ast$ that parameterize action choices.

We assume that the noise variables are ``well-behaved'' in accordance with the following assumption

\begin{assumption}
\label{ass:noise}
We assume that, for any $t \geq 1$, the noise variables $\epsilon_t \in \R^d$ and $\xi_t \in \R$ are $\sigma$-subGaussian and $\eta$-subGaussian, respectively. That is,
$$
\log\E\exp\left\{\langle \lambda, \epsilon_t\rangle\right\} \leq \frac{\|\lambda\|^2\sigma^2}{2}, \forall \lambda \in \R^d\quad \text{and} \quad \log\E\exp\left\{\lambda \xi_t\right\} \leq \frac{\lambda^2\eta^2}{2}, \forall \lambda \in \R.
$$

Further, we assume there is some constant $\gamma > 0$ such that
$$
\left\|\E\left[\epsilon_t\epsilon_t^T\right]\right\|_{2} \leq \gamma, \forall t \geq 1.
$$

\end{assumption}

The goal of the agent is to minimize, with high probability, a quantity called \textbf{regret}, which measures the performance of an action selection policy with respect to an optimal policy. More specifically, in this work we consider three notions of regret, which we call the \textit{weak regret}, \textit{intermediate regret}, and \textit{strong regret}. These quantities are defined respectively as
$$
R_T^w := \sum_{t = 1}^T \langle \theta(a^\ast_t), Z_t \rangle - \langle \theta(a_t), Z_t\rangle,
$$
$$
R_T^i := \sum_{t = 1}^T \langle \theta(a^\ast_t), X_t \rangle - \langle \theta(a_t), X_t\rangle,
$$
and
$$
R_T^s := \sum_{t = 1}^T \langle \theta(a^\square_t), X_t \rangle - \langle \theta(a_t), X_t \rangle.
$$

In the above $a^\ast_t := \arg\max_{a \in [A]}\langle \theta(a), Z_t\rangle$ is the optimal action for a policy that knows all true slope vectors, but can only de-noise the context $Z_t$ up to the proportion of the noise that lies in the low-dimensional subspace $W^\ast$. Given the independence of noise presented in Assumption~\ref{ass:noise}, $a^\ast_t$ can be viewed as the action that a policy consistently estimating the slope vectors $\theta(a)$ would take after receiving sufficiently many samples. Likewise, $a^\square := \arg\max_{a \in [A]}\langle \theta(a), X_t\rangle$ is the optimal action that an omniscient adversary knowing both the slope vectors $\theta(a)$ and the true contexts $X_t$ would take. 


We further impose the following assumptions on the problem.


\begin{assumption}[\textbf{Slope Bounds}]
\label{ass:bounded_slope}
We assume that there exists some constant $L > 0$ such that $\|\theta(a)\|_2 \leq L$ for all $a \in [A]$. 
\end{assumption}

\begin{assumption}[\textbf{Context Upper Bounds}]
We assume that, for any $t \geq 1$, we have $X_t = O(\sqrt{d})$.
    
\end{assumption}

We do not leverage the following assumptions in the construction of our confidence bounds. We will, however, need the following assumptions in our regret analysis. 

\begin{assumption}[\textbf{Well-Distributed Slope Vectors}]
For any $t \geq 1$, there exists an action $a \in [A]$ such that $\langle \theta(a), X_t\rangle = \Omega(\sqrt{d})$.

\end{assumption}

\subsection{Notation and Linear Algebraic Prerequisites}

\subsubsection{Data-Dependent Quantities}
For $t \geq 1$, we define the matrix $\vZ_t \in \R^{t \times d}$ to be the matrix with $Z_1, \dots, Z_t$ as its rows. $\vX_t = (X_1, \dots, X_t)^T \in \R^{t \times d}, \Epsilon_t = (\epsilon_1, \dots, \epsilon_t)^T \in R^{t \times d}, \vY_t \in \R^{t \times 1},$ and $\Xi_t = (\xi_1, \dots, \xi_t)^T \in \R^{t \times 1}$ are defined similarly.

For any action $a \in [A],$ let $N_t(a) := \{s \leq t : a_s = a \}$ be the set of rounds up to and including time $t$ on which action $a$ was chosen. Likewise, let $n_t(a) := |N_t(a)|$ denote the number of rounds by round $t$ on which action $a$ was selected.

For $a \in [A]$, let us enumerate in increasing order $N_t(a)$ as $i_1 \leq \cdots \leq i_{n_t(a)}$. We define $\vZ_t(a) \in \R^{n_t(a) \times d}$ to be $\vZ(a) = (Z_{i_1}, \dots, Z_{i_{n_t(a)}})^T$, and define $\vX_t(a), \Epsilon_t(a), \vY_t(a),$ and $\Xi_t(a)$ entirely analogously.

For a given regularization parameter $\rho > 0$ and action $a \in [A]$, we define the covariance matrix associated with action $a$ up to time $t$ as
$$
\cV_t(a) := \vZ_t(a)^T\vZ_t(a) + \rho I_d.
$$
With this covariance matrix, we can define the ridge estimate of the unknown slope vector $\theta(a)$ as 
$$
\theta_t(a) := \cV_t(a)^{-1}\vZ_t(a)^T\vY_t(a).
$$


\subsubsection{Subspaces and Projection Matrices}
Let $W \subset \R^d$ be a fixed linear subspace with $\dim(W) = r$, and let $\vW \in \R^{d \times r}$ be a matrix whose columns form an orthonormal basis for $W$. Given such an orthonormal basis, we can identify the subspace $W$ with the projection matrix $\vP^W := \vW\vW^T$.

We define the projection of $\vZ_t(a)$ and $\vX_t(a)$ onto $W$ as $\vZ_t^W(a) := \vZ_t(a)\vP^W$ and $\vX_t^W(a) := \vX_t(a)\vP^W$, respectively. For $\cV_t(a)$ as defined above, we can define the projection of $\cV_t(a)$ onto $W$ as 
$$
\cV_t^W(a) := \vZ_t^W(a)^T\vZ_t^W(a) + \rho I_W.
$$
Likewise, we can define the estimate of $\theta(a)$ projected onto the subspace $W$ as
$$
\theta_t^W(a) := \cV_t^W(a)^{-1}\vZ_t^W(a)^T\vY_t(a).
$$

\subsubsection{Singular Value Decomposition}

Any matrix $\vA \in \R^{t \times d}$ can be written in its singular value decomposition $\vA = \vU \Sigma \vV^T$, where $\vU \in \R^{t \times d\land t}$ and $\vV \in \R^{d \times d \land t}$ are matrices with orthonormal columns, and $\Sigma = \diag(\sigma_1(\vA), \dots, \sigma_{d \land t}(\vA)) \in \R^{(d \land t) \times (d \land t)}$ is a diagonal matrix containing the singular values of $\vA$, where we assume $\sigma_1(\vA) \geq \dots \geq \sigma_{n \land t}(\vA) \geq 0$. From the singular value decomposition for a matrix $\vA$ and for a truncation level $k$, we can define the truncation of $\vA$ onto its top $k$ principal components as $\vA_{k} := \vU_{k} \diag(\sigma_1(\vA), \dots, \sigma_{k \land d \land t}(\vA))\vV^T_k$, where $\vU_k \in \R^{t \times k \land d \land t}$ is the matrix with the first $k \land d \land t$ columns of $\vU$, and $\vV \in \R^{n \times k \land d \land t}$ is defined analogously. Given such a singular value decomposition, we can define the projection matrix onto the subspace spanned by the top $k$ right singular vectors as $\vP_{k} \in \R^{d \times d }$ given by $\vP_k := \vV_{k}\vV_k^T$.

For $t \geq 1$ and $\vZ_t$ and $\vX_t$ as defined above, let us write their $r$-truncated singular value decompositions as $\vZ_{t, r} = \wh{\vU}_{t, r}\diag(\sigma_1(\vZ_t), \dots, \sigma_{r \land t \land n}(\vZ_t))\wh{\vV}^T_{t, r}$ and $\vX_{t, r} = \wc{\vU}_{t, r}\diag(\sigma_1(\vX_t), \dots, \sigma_{r \land t \land n}(\vZ_t))\wc{\vX}^T_{t, r}$, and the corresponding projections onto the top $r$ right singular vectors of $\vZ$ and $\vX$ as $\wh{\vP}_t$ and $\wc{\vP}_t$, respectively. In line with our previous discussion on projection matrices, for $a \in [A]$ and $t \in [T]$, we define $\wh{\vZ}_t(a) := \vZ_t(a)\wh{\vP}_t$, $\wh{\vX}_t(a) := \vX_t(a)\wh{\vP}_t, \wh{\cV}_t(a) := \wh{\vZ}_t(a)^T\wh{\vZ}_t(a) + \rho \wh{\vP}_t,$ and $\wh{\theta}_t(a) := \wh{\cV}_t(a)^{-1}\wh{\vZ}_t(a)\vY_t(a)$. We define the ``checked'' quantities $\wc{\vZ}_t(a), \wc{\vX}_t(a), \wc{\cV}_t(a),$ and $\wc{\theta}_t(a)$ exactly analogously with respect to the projection matrix $\wc{\vP}_t$. 

\subsubsection{Signal to Noise Ratio}

Lastly, we touch on the notion of a signal-to-noise ratio, which will be an integral component of our regret analysis in the following section. At a high level, the signal-to-noise ratio captures how strongly the signal induced by the true covariates $X_t$ can be detected through the noise variables $\epsilon_t$. Recall that, for any $t \geq 1$, the matrix $\vX_t \in \R^{t \times d}$ has $X_1, \dots, X_t$ as its columns. Since, for any $t$, $X_t \in W^\ast$, we know that the rank $\vX_t$ is at most $r$, and hence $\sigma_k(\vX_t) = 0$ for all $k > r$. Thus, $\sigma_r(\vX_t)$ is the smallest singular value of $\vX_t$ that has potentially positive value. Using this value, we define the $(\delta, \rho)$-signal-to-noise ratio at time $t \geq 1$ to be the quantity $s_t$ given by
$$
\snr_t := \frac{\sigma_r(\vX_t)}{\sigma\left(\sqrt{d} + \sqrt{t} + \log\left(\frac{t(t + 1)}{\delta}\right)\right)}.
$$
The denominator provides a time-uniform upper bound of the behavior of the operator norm of $\Epsilon_t$, as with high probability, simultaneously for all $t \geq 1$, we have $\|\Epsilon_t\|_{op} \leq C\sigma\left(\sqrt{d} + \sqrt{t} + \log\left(\frac{t(t + 1)}{\delta}\right)\right)$ for some absolute constant $C > 0$.  

We can equivalently define the signal-to-noise ratio with respect to a fixed action $a \in [A]$. We define this quantity as
$$
\snr_t(a) := \frac{\sigma(\vX_t(a))}{\sigma\left(\sqrt{d} + \sqrt{n_t(a)} + \log\left(\frac{n_t(a)(n_t(a) + 1)}{\delta}\right)\right)}.
$$

Note that the signal to noise ratio, as defined above, depends on the \textit{true} covariates $X_1, \dots, X_t$. A more practical quantity of interest for the agent is the \textbf{random signal to noise ratio}, which are defined as
$$
\wh{\snr}_t := \frac{\sigma_r(\wh{\vZ}_t)}{\sigma\left(\sqrt{d} + \sqrt{t} + \log\left(\frac{t(t + 1)}{\delta}\right)\right)}
$$
in the general sense and
$$
\wh{\snr}_t(a) := \frac{\sigma(\wh{\vZ}_t(a))}{\sigma\left(\sqrt{d} + \sqrt{n_t(a)} + \log\left(\frac{n_t(a)(n_t(a) + 1)}{\delta}\right)\right)}
$$
in the action-specific. In the sequel, it will be of interest ot study how $\wh{\snr}_t$ concentrates around $\snr_t$ under various assumptions on the covariates.


\begin{comment}
\subsection{Principal Component Regression UCB}

We now define the primary algorithm we will use to solve the bandits with noisy contexts problems: the Principal Component Regression Upper Confidence Bound algorithm, or PCR-UCB for short. At a high level, the maintains estimates for each of the unknown slope vectors $\theta(a), \dots, \theta(A) \in W^\ast \subset \R^d$, along with an estimate projection operator onto the unknown, low-dimensional subspace $W^\ast$. At each round, the algorithm chooses the action that has the highest upper bound on reward potential. The algorithm then receives corresponding feedback, and updates the estimate of the slope vector for the action that was played, and the estimate for the underlying, low-dimensional subspace. We present the PCR-UCB algorithm in full detail in Algorithm~\ref{alg:PCR-UCB}.


\begin{algorithm}

\caption{Principal Component Regression Upper Confidence Bound}
\begin{algorithmic}[0]
\Require 
\Function{PCR-UCB}{$(C_t)$, $\rho$, $T$}
\For{$t \in 1, \dots, T$}
    \State Compute $\wh{\vP}_t := \wh{\vV}_{t, r} \wh{\vV}^T_{t, r}$.
    \State Compute $\wh{\theta}_t(a) := \wh{\cV}_t(a)^{-1}\wh{\vZ}_t(a)^T\vY_t(a)$ for $a\in [A]$.
    \State Observe $Z_t := X_t + \epsilon_t$
    \State Play $a_t := \arg\max_{a \in [A]}\max_{\theta \in C_t(a, \wh{\theta}_t(a), \wh{\vP}_t)}\langle \theta, Z_t\rangle$
    \State Observe reward $Y_t := \langle \theta(d_t), X_t\rangle + \xi_t$

\EndFor
\State \Return


\EndFunction

\end{algorithmic}
\label{alg:PCR-UCB}
\end{algorithm}
\end{comment}

\subsection{Constructing Confidence Sets}

In this section 

\begin{lemma}[\textbf{Error bound in true subspace}]
\label{lem:ellipsoid}
Let $\delta \in (0, 1)$ be an arbitrary confidence parameter. Then, there is a universal constant $C_1 > 0$ such that, with probability at least $1 - \delta$, simultaneously for all $t \in [T]$ and $a \in [A]$, we have 
\begin{align*}
&\left\|\wc{\cV}_t(a)^{1/2}\left(\wc{\theta}_t(a) - \theta(a)\right)\right\|_2 \leq \sqrt{\rho}L + \eta\sqrt{2\log\left(\frac{A}{\delta}\right) + r\log\ell_t(a, \rho, \delta)} \\
&+  LC_2\sigma(\gamma \lor 1)\left(\sqrt{r} + \sqrt{n_t}  +\sqrt{\log\left(\frac{An_t(n_t + 1)}{\delta}\right)}\right) 
\end{align*}
where we have let $n_t := n_t(a)$ and 
$$
\ell_t(a, \rho, \delta) := 1 + \frac{C\sigma(\gamma \lor 1)\left(\sqrt{n_t} + \sqrt{r} + \sqrt{\log\left(\frac{An_t(n_t + 1)}{\delta}\right)}\right)^2}{\rho}
$$
for notational ease.
\end{lemma}

\begin{proof}
First, by Lemma~\ref{lem:int:diff}, we see that we have, for any $a \in [A]$ and $t \in [T]$
$$
\wc{\theta}_t(a) - \theta(a) = \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\Xi_t(a) + \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\wc{\Epsilon}_t(a) - \rho\wc{\cV}_t(a)^{-1}\theta(a).
$$
With this decomposition in hand, we can use the triangle inequality for norms to see.
Using this decomposition in conjunction with the triangle inequality for norms, we have that
\begin{align*}
&\left\|\wc{\cV}_t(a)^{1/2}\left(\wc{\theta}_t(a) - \theta(a)\right)\right\|_2 \\
&\leq \left\|\wc{\cV}_t(a)^{-1/2}\wc{\vZ}_t(a)^T\Xi_t(a)\right\|_2 + \rho\left\|\wc{\cV}_t(a)^{-1/2}\theta(a)\right\|_2 + \left\|\wc{\cV}_t(a)^{-1/2}\wc{\vZ}_t(a)^T\wc{\Epsilon}_t(a)\theta(a)\right\|_2 \\
&\leq \left\|\wc{\cV}_t(a)^{-1/2}\wc{\vZ}_t(a)^T\Xi_t(a)\right\|_2 + \sqrt{\rho}L + \left\|\wc{\cV}_t(a)^{-1/2}\wc{\vZ}_t(a)^T\wc{\Epsilon}_t(a)\theta(a)\right\|_2.
\end{align*}

We bound the first and last terms separately. Applying Lemma~\ref{lem:int:mixture} for each $a \in [A]$ and taking a union bound over actions yields that, with probability at least $1 - \delta$, simultaneously for all $t \in [T]$ and $a \in [A]$,
\begin{align*}
\left\|\wc{\cV}_t(a)^{-1/2}\wc{\vZ}_t(a)^T\Xi_t(a)\right\|_2 &\leq \eta\sqrt{2\log\left(\frac{A}{\delta}\sqrt{\det\left(\rho^{-1}\wc{\cV}_t(a)\right)}\right)} \\
&\leq \eta\sqrt{2\left[\log\left(\frac{A}{\delta}\right) +  r\log\left(1 + \frac{\sigma_1(\wc{\vZ}_t(a))^2}{\rho}\right)\right]} \\
&\hspace{-1.5cm}\leq \eta\sqrt{2\left[\log\left(\frac{A}{\delta}\right) + r\log\left(1 + \frac{C\sigma(\gamma \lor 1)\left(\sqrt{n_t} + \sqrt{r} + \sqrt{\log\left(\frac{An_t(n_t + 1)}{\delta}\right)}\right)^2}{\rho}\right)\right]} \\
&= \eta\sqrt{2\log\left(\frac{A}{\delta}\right) + r\log \ell_t(a, \rho, \delta)}
.
\end{align*}
Next, observe that
\begin{align*}
\left\|\wc{\cV}_t(a)^{-1/2}\wc{\vZ}_t(a)^T\wc{\Epsilon}_t(a)\theta(a)\right\|_2 &\leq \left\|\wc{\cV}_t(a)^{-1/2}\wc{\vZ}_t(a)^T\right\|_{op}\left\|\wc{\Epsilon}_t(a)\right\|_{op}\left\|\theta(a)\right\|_2.
\end{align*}
First, note that $\|\theta(a)\|_2 \leq L$ by assumption. Next, Lemma~\ref{lem:int:term_bd} yields
$$
\left\|\wc{\cV}_t(a)^{-1/2}\wc{Z}_t(a)^T\right\|_{op} \leq 1.
$$
Lastly, by taking a union bound over $t \in [T]$ and $a \in [A]$ and applying Lemma~\ref{lem:int:cov_noise} coupled with Lemma~\ref{lem:ext:subg}, we see that there exists some absolute constants $C_1, C_2 > 0$ such that, with probability at least $1 - \delta$, simultaneously for all $t \geq 1$ and $a \in [A]$, we have, by 
\begin{align*}
\left\|\wc{\Epsilon}_t(a)\right\|_{op} &\leq C_1\sigma\sqrt{\left(\sqrt{r} + \sqrt{\log\left(\frac{An_t(n_t + 1)}{\delta}\right)}\right)\left\{\sqrt{n_t} + \sqrt{r} + \sqrt{\log\left(\frac{An_t(n_t + 1)}{\delta}\right)}\right\} + n_t\gamma} \\
&\leq C_2\sigma(\gamma \lor 1)\left(\sqrt{r} + \sqrt{n_t} + \sqrt{\log\left(\frac{An_t(n_t + 1)}{\delta}\right)}\right).
\end{align*}
where we have let $n_t := n_t(a)$ for notational simplicity. Combining these bounds gives the desired result.
\end{proof}




\begin{theorem}[\textbf{Simpler Confidence Set}]
\label{thm:conf_ball}
Let $\delta \in (0, 1)$ be an arbitrary confidence parameter. Then, there there are universal constants $C_1, C_2 > 0$ such that, with probability at least $1 - O(\delta)$, simultaneously for all $t \geq 1$ and $a \in [A]$, we have
\begin{align*}
\left\|\wh{\theta}_t(a) - \theta(a)\right\|_2 &\leq \frac{LC_1\sigma(\gamma \lor 1)}{\wh{\snr}_t}\left(1 + \frac{LC_2\sigma(\gamma \lor 1)}{\wh{\snr}_t(a)}\right) + \frac{LC_1\sigma(\gamma \lor 1)}{\wh{\snr}_t(a)} \\
&+ \frac{1}{\sigma_r(\wh{\vZ}_t(a))}\left(\sqrt{\rho}L + \eta\sqrt{2\log\left(\frac{A}{\delta}\right) + r\log\ell_t(a, \rho, \delta)}\right)
\end{align*}

\end{theorem}
 
\begin{proof}
Observe first that we can write
$$
\wh{\theta}_t(a) - \theta(a) = \wh{\vP}_t(\wh{\theta}_t(a) - \theta(a)) + (\wc{\vP}_t^{\perp} - \wh{\vP}_t^{\perp})\theta(a).
$$
Using this decomposition, we have, via the triangle inequality
$$
\left\|\wh{\theta}_t(a) - \theta(a)\right\| \leq \left\|\wh{\vP}_t(a)(\wh{\theta}_t(a) - \theta(a))\right\| + \left\|(\wh{\vP}_t^{\perp} - \wc{\vP}_t^{\perp})\theta(a)\right\|.
$$
We bound these two terms separately. For the second, observe that we have, with probability at least $1 - \delta$, simultaneously for all $t \geq 1$
\begin{align*}
\left\|(\wh{\vP}_t^{\perp}  - \wc{\vP}_t^{\perp})\theta(a)\right\|_2 & \leq \left\|\wh{\vP}_t^{\perp} - \wc{\vP}_t^{\perp}\right\|_{op}\left\|\theta(a)\right\| \\
&\leq L \left\|\wh{\vP}_t^{\perp} - \wc{\vP}_t^{\perp}\right\|_{op} = L \left\|\wh{\vP}_t - \wc{\vP}_t\right\|_{op} \\
&\leq \frac{2LC_1(\gamma \lor 1)\left(\sqrt{d} + \sqrt{t} + \sqrt{\log\left(\frac{t(t + 1)}{\delta}\right)}\right)}{\sigma_r(\wh{\vZ}_t(a))}.
\end{align*}
Next, for the first term, observe that we have
\begin{align*}
\left\|\wh{\vP}_t\left(\wh{\theta}_t(a) - \theta(a)\right)\right\|_2 &\leq \frac{1}{\sigma_r(\wh{\vZ}_t(a))}\left\|\wh{\vZ}_t\left(\wh{\theta}_t(a) - \theta(a)\right)\right\|_2 \\
&\leq \frac{1}{\sigma_r(\wh{\vZ}_t(a))}\left[\underbrace{\left\|\wh{\vZ}_t(a)\wh{\theta}_t(a) - \vX_{t}(a)\theta(a)\right\|_2}_{T_1} + \underbrace{\left\|\vX_t(a) \theta(a) - \wh{\vZ}_t(a)\theta(a)\right\|_2}_{T_2}\right]
\end{align*}
We now bound $T_1$ and $T_2$ separately. Starting with $T_1$, we see
\begin{align*}
T_1 &:= \left\|\wh{\vZ}_t(a)\wh{\theta}_t(a) - \vX_{t}(a)\theta(a)\right\|_2 \\
&= \left\|\wh{\vZ}_t(a)\wh{\theta}_t(a) - \vX_{t}(a)\theta(a) + \Xi_t(a) - \Xi_t(a)\right\|_2\\
&\leq \left\|\wh{\vZ}_t(a)\wh{\theta}_t(a) - \vY_t(a)\right\|_2 + \left\|\Xi_t(a)\right\|_2 \\
&\leq \left\|\wc{\vZ}_t(a)\wc{\theta}_t(a) - \vY_t(a)\right\|_2 + \left\|\Xi_t(a)\right\|_2 \\
&\leq \left\|\wc{\vZ}_t(a)\wc{\theta}_t(a) - \vX_t(a)\theta(a)\right\|_2 + 2\left\|\Xi_t(a)\right\| \\
&\leq \left\|\wc{\vZ}_t(a)\left(\wc{\theta}_t(a) + \theta(a)\right)\right\|_2 + 2\left\|\Xi_t(a)\right\|_2 + \left\|\wc{\Epsilon}_t(a)\theta(a)\right\|_2 \\
&\leq \left\|\wc{\cV}_t(a)^{1/2}\left(\wc{\theta}_t(a) - \theta(a)\right)\right\|_2 + 2 \left\|\Xi_t(a)\right\|_2 + L\left\|\wc{\Epsilon}_t(a)\right\|_{op}.
\end{align*}
Next, we bound $T_2$. We have
\begin{align*}
T_2 &:= \left\|\vX_t(a) \theta(a) - \wh{\vZ}_t(a)\theta(a)\right\|_2 \\
&\leq \left\|\wc{\vZ}_t(a)\theta(a) - \wh{\vZ}_t(a)\theta(a)\right\|_2 + \left\|\wc{\Epsilon}_t(a)\theta(a)\right\|_2 \\
&= \left\|\vZ_t(a)(\wc{\vP}_t - \wh{\vP}_t)\theta(a)\right\|_2 + \left\|\wc{\Epsilon}_t(a)\theta(a)\right\|_2 \\
&\leq L(\|\vX_t(a)\|_2 + \|\Epsilon_t(a)\|_2)\left\|\wc{\vP}_t - \wh{\vP}_t\right\|_{op} + L\left\|\wc{\Epsilon}_t(a)\right\|_{op}.
\end{align*}
Thus, in sum, we have the bound
\begin{align*}
\left\|\wh{\theta}_t(a) - \theta(a)\right\|_2 &\leq L\left\|\wh{\vP}_t - \wc{\vP}_t\right\|_{op}\left(1 + \frac{\left\|\vX_t(a)\right\|_{op} + \left\|\Epsilon_t(a)\right\|_{op}}{\sigma_r(\wh{\vZ}_t(a))}\right) \\
&+ \frac{1}{\sigma_r(\wh{\vZ}_t(a))}\left(\left\|\wc{\cV}_t(a)^{1/2}\left(\wc{\theta}_t(a) - \theta(a)\right)\right\|_2 + 2\left\|\Xi_t(a)\right\|_2 + 2L\left\|\wc{\Epsilon}_t(a)\right\|_{op}\right) \\
&\hspace{-1.5cm}\leq L C_1 \sigma (\gamma \lor 1)\left(\frac{\sqrt{d} + \sqrt{t} + \sqrt{\log\left(\frac{At(t + 1)}{\delta}\right)}}{\sigma_r(\wh{\vZ}_t)}\right)\left(1 + \frac{LC_1\sigma(\gamma \lor 1)\left(\sqrt{t} + \sqrt{d} + \sqrt{\log\left(\frac{An_t(n_t + 1)}{\delta}\right) + LC_2\sqrt{dt}}\right)}{\sigma_r(\wh{\vZ}_t(a))}\right) \\
&\hspace{-2.5cm}+ \frac{1}{\sigma_r(\wh{\vZ}_t(a))}\left(\sqrt{\rho}L + \eta\sqrt{2\log\left(\frac{A}{\delta}\right) + r\log\ell_t(a, \rho, \delta)} 
    +  LC_1\sigma(\gamma \lor 1)\left(\sqrt{r} + \sqrt{n_t}  +\sqrt{\log\left(\frac{An_t(n_t + 1)}{\delta}\right)}\right)\right) \\
    &= \frac{LC_1\sigma(\gamma \lor 1)}{\wh{\snr}_t}\left(1 + \frac{LC_1\sigma(\gamma \lor 1)}{\wh{\snr}_t(a)} + C_2 L \frac{LC_2\sqrt{dt}}{\sigma_r(\wh{\vZ}_t(a))}\right) + \frac{LC_1\sigma(\gamma \lor 1)}{\wh{\snr}_t(a)} \\
    &+ \frac{1}{\sigma_r(\wh{\vZ}_t(a))}\left(\sqrt{\rho}L + \eta\sqrt{2\log\left(\frac{A}{\delta}\right) + r\log\ell_t(a, \rho, \delta)}\right) 
\end{align*}
\end{proof}

\begin{corollary}[\textbf{Next Sample Prediction Error}]
Let $\delta \in (0, 1)$ be arbitrary. We have, with probability at least $1 - O(\delta)$, simultaneously for all $t \geq 1$ and $a \in [A]$,
\[
\left(\langle \wh{\theta}_{t}(a), Z_{t + 1}\rangle - \langle \theta(a), X_{t + 1}\rangle\right)^2 \leq 
\]
\end{corollary}

\begin{proof}
Observe first that we have
\[
\langle \wh{\theta}_{t}(a), Z_{t + 1} \rangle - \langle \theta(a), X_{t + 1} \rangle = \langle \wh{\theta}_{t}(a), \epsilon_{t + 1} \rangle + \langle \wh{\theta}_{t}(a) - \theta(a), X_{t + 1}\rangle.
\]
Thus, we have, with probability at least $1 - O(\delta)$, simultaneously for all $a \in [A]$ and all $t \geq 1$,
\begin{align*}
\left(\langle \wh{\theta}_{t}(a), Z_{t + 1}\rangle - \langle \theta(a), X_{t + 1}\rangle\right)^2 &\leq 2\langle\wh{\theta}_{t}(a), \epsilon_{t + 1} \rangle^2 + 2\langle \wh{\theta}_{t}(a) - \theta(a), X_{t + 1}\rangle^2 \\
&\leq 4L^2\sigma^2\log\left(\frac{t(t + 1)}{\delta}\right)
\end{align*}

\end{proof}
\begin{comment}
\begin{theorem}

\end{theorem}

\begin{proof}
We proceed much in the same way as the preceding theorem, taking a different approach to bounding the term $\left\|\wh{\vP}_t\left(\wh{\theta}_t(a) - \theta(a)\right)\right\|_{2}$. We have
\begin{align*}
\left\|\wh{\vP}_t\left(\wh{\theta}_t(a) - \theta(a)\right)\right\|_2 &\leq \frac{1}{\sqrt{\sigma_r(\wh{\vZ}_t(a)) + \rho}}\left\|\wh{\cV}_t(a)^{1/2}\left(\wh{\theta}_t(a) - \theta(a)\right)\right\|_2 \\
&\frac{1}{\sqrt{\sigma_r(\wh{\vZ}_t(a)) + \rho}}\Bigg( \underbrace{\left\|\left(\wh{\cV}_t(a)^{1/2} - \left(\wh{\vZ}_t(a)^T\wh{\vZ}_t(a)\right)^{1/2}\right)\wh{\theta}_t(a)\right\|_2}_{T_1} \\
&\hspace{-1cm}+ \underbrace{\left\|\left(\wh{\vZ}_t(a)^T\wh{\vZ}_t(a)\right)^{1/2} \left(\wh{\theta}_t(a) - \theta(a)\right)\right\|_2}_{T_2} + \underbrace{\left\|\left(\wh{\cV}_t(a)^{1/2} - \left(\wh{\vZ}_t(a)^T\wh{\vZ}_t(a)\right)^{1/2}\right)\theta(a)\right\|_2}_{T_3}\Bigg)
\end{align*}

Observe that we have
\begin{align*}
T_1 &= \left\|\left(\wh{\cV}_t(a)^{1/2} - \left(\wh{\vZ}_t(a)^T\wh{\vZ}_t(a)\right)^{1/2}\right)\wh{\theta}_t(a)\right\|_2 \\
&\leq \left\|\wh{\cV}_t(a)^{1/2} - \left(\wh{\vZ}_t(a)^T\wh{\vZ}_t(a)\right)^{1/2}\right\|_{op}\left\|\wh{\theta}_t(a)\right\|_2 \\
&\leq \sqrt{\rho}R_\rho.
\end{align*}
An identical argument gives $T_3 \leq \sqrt{\rho} L$. Lastly, observe we have
\[
T_2 = \left\|\left(\wh{\vZ}_t(a)^T\wh{\vZ}_t(a)\right)^{1/2} \left(\wh{\theta}_t(a) - \theta(a)\right)\right\|_2 = \left\|\wh{\vZ}_t(a)^{1/2}\left(\wh{\theta}_t(a) - \theta(a)\right)\right\|_2,
\]
and we know how to bound the right hand side quantity from the proof of the previous Theorem. Piecing things together, we have that
\end{proof}
\end{comment}



==> arxiv/internal_technical_lemmas.tex <==
\section{Internal Technincal Lemmas}

In this section, we provide several technical lemmas that will be used in the main proofs in this paper. We present these lemmas separately in this section so that, at least in the drafting phase, our proofs are more modular.

\begin{lemma}
\label{lem:int:proj_close}
There is a constant $C > 0$ such that, for any $t \geq 1$ and $\delta \in (0, 1)$, we have, with probability at least $1 - \delta$, 
$$
\left\|\wh{\vP}_t - \wc{\vP}_t\right\|_{op} \leq \frac{2C\sigma(\gamma \lor 1)\left(\sqrt{d} + \sqrt{t} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)}{\sigma_r(\wh{\vZ}_t)}.
$$
\end{lemma}

\begin{proof}
Recall that we can write
$$
\wh{\vP}_t = \wh{\vV}_{t, r}\wh{\vV}_{t, r}^T \quad \text{and} \quad \wc{\vP}_t = \wc{\vV}_{t, r}\wc{\vV}_{t, r}^T,
$$
where we have again the singular value decompositions
$$
\vZ_t = \wh{\vV}_t\wh{\Sigma}_t\wh{\vU}_t \quad \text{and} \quad \vX_t = \wc{\vU}_t\wc{\Sigma}_t\wc{\vV}_t^T.
$$
Now, applying Lemma~\ref{lem:ext:wedin} and Lemma~\ref{lem:int:cov_noise}, we have that
\begin{align*}
\left\|\wh{\vP}_t - \wc{\vP}_t\right\|_{op} &= \left\|\wh{\vV}_{t, r}\wh{\vV}_{t, r}^T  - \wc{\vV}_{t, r}\wc{\vV}_{t, r}^T\right\|_{op} \\
&\leq \frac{2\left\|\vX_t - \vZ_t\right\|_{op}}{\sigma_r(\wh{\vZ}_t)}  \\
&= \frac{2\|\Epsilon_t\|_{op}}{\sigma_r(\wh{\vZ}_t)} \\
&\leq \frac{2C\sigma(\gamma \lor 1)\left(\sqrt{d} + \sqrt{t} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)}{\sigma_r(\wh{\vZ}_t)}.
\end{align*}
This proves the desired result.
\end{proof}

\begin{lemma}
\label{lem:int:term_bd}
Let $\vA \in \R^{t \times d}$ be a matrix, and let $\rho > 0$ be arbitrary. Suppose $\vA$ has $1 \leq k \leq t \land d$ non-zero singular values. Then,
$$
\left\|(\vA^T\vA + \rho I_d)^{-1/2}\vA^T\right\| \leq \frac{\sigma_k(\vA)}{\sqrt{\sigma_k(\vA)^2 +\rho}} \leq 1
$$

\end{lemma}

\begin{proof}
    Let us write the singular value decomposition of $\vA$ as
    $$
    \vA = \vU \Sigma \vV^T = \vU_k \Sigma_k \vV_k^T,
    $$
    where the second equality follows from the fact that $\vA$ has exactly $k$ non-zero singular values. We have the equality
    $$
    \vA^T\vA + \rho I_d = \vV (\Sigma_k^2 + I_k) \vV^T_k.
    $$
    Thus, we see
    \begin{align*}
    \left\|(\vA^T\vA + \rho I_d)^{-1/2}\vA^T\right\|_{op} &= \left\|\vV_k (\Sigma_k^2 + \rho I_k)^{-1/2}\vV_k^T \vV_k^T\vV_k \Sigma_k \vU_k^T\right\|_{op} \\
    &= \left\|(\Sigma_k^2 + \rho I_k)^{-1/2}\Sigma_k\right\|_{op} \\
    &= \max_{i = 1}^k \frac{\sigma_i(\vA)}{\sqrt{\rho + \sigma_i(\vA)^2}} \leq \frac{\sigma_k(\vA)}{\sqrt{\rho + \sigma_k(\vA)^2}}.
    \end{align*}
    The last inequality in the lemma statement is trivial.
\end{proof}

\begin{lemma}
\label{lem:int:diff}
Recall that, for any $t \in [T]$ and $a \in [A],$ we have defined the estimate of $\theta(a)$ under $\wc{\vP}_t$ to be
$$
\wc{\theta}_t(a) := \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\vY_t(a).
$$
We have
$$
\wc{\theta}_t(a) - \theta(a) = \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\Xi_t(a) + \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\wc{\Epsilon}_t(a) - \rho\wc{\cV}_t(a)^{-1}\theta(a).
$$
\end{lemma}

\begin{proof}
A straightforward computation yields
\begin{align*}
\wc{\theta}_t(a) - \theta(a) &= \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\vY_t(a) - \theta(a) \\
&= \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)(\vX_t(a)\theta(a) + \Xi_t(a)) - \theta(a) \\
&=  \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)\vX_t(a)\theta(a) + \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\Xi_t(a) -\theta(a) \\
&\qquad \pm \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)\wc{\Epsilon}_t(a) \pm \rho\wc{\cV}_t(a)^{-1}\theta(a)\\
&= \wc{\cV}_t(a)^{-1}\left[\wc{\vZ}_t(a)^T(\vX_t(a) + \wc{\Epsilon}_t(a)) + \rho I_d\right]\theta(a) + \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\Xi_t(a) - \theta(a) \\
&\qquad - \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)\wc{\Epsilon}_t(a) - \rho\wc{\cV}_t(a)^{-1}\theta(a)\\
&= \wc{\cV}_t(a)^{-1}\left[\wc{\vZ}_t(a)^T\wc{\vZ}_t(a) + \rho I_d\right]\theta(a) + \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\Xi_t(a) - \theta(a) \\
&\qquad - \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)\wc{\Epsilon}_t(a) - \rho\wc{\cV}_t(a)^{-1}\theta(a)\\
&= \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\Xi_t(a) - \wc{\cV}_t(a)^{-1}\wc{\vZ}_t(a)^T\wc{\Epsilon}_t(a) - \rho\wc{\cV}_t(a)^{-1}\theta(a),
\end{align*}
which proves the desired result.
\end{proof}

\begin{lemma}[\textbf{Covariance Noise Bound}]
\label{lem:int:cov_noise}
Let $W \subset \R^d$ be an arbitrary subspace with $\dim(W) = r$. Assume $\phi_1, \dots, \phi_t \in \R^d$ are independent random vectors such that (i) $\|\phi_i\|_{\psi_2} \leq K$ and (ii) $\|\E\phi_i\phi_i^T\|_{op} \leq \gamma$, for all $i \in [t]$. Define $\Phi_t := (\phi_1, \dots, \phi_t)^T$. Let $\delta \in (0, 1)$ be an arbitrary confidence parameter. Then, there are constants $C_1, C_2 > 0$ such that, with probability at least $1 - \delta$, we have 
\begin{align*}
\left\|\Phi_t^W\right\|_{op} &\leq  C_1K\sqrt{\left(\sqrt{r} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)\left\{\sqrt{t} + \sqrt{r} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right\} + t\gamma} \\
&\leq C_2K(\gamma\lor1)\left(\sqrt{r} + \sqrt{t} + \log\left(\frac{1}{\delta}\right)\right)
\end{align*}

\end{lemma}

\begin{proof}
By definition, we have
$$
\Phi_t^W = \Phi_t \vP^W = \Phi_t \vW \vW^T,
$$
where $\vW \in \R^{d \times r}$ is a matrix whose columns form an orthonormal basis for $W$.  Thus, we have that
$$
\|\Phi_t^W\|_{op} = \|\Phi_t \vW \vW^T\|_{op} = \|\Phi_t \vW\|_{op}.
$$
Let $\wt{\Phi}_t \in \R^{t \times r}$ be given by $\wt{\Phi}_t := \Phi_t \vW$. Correspondingly, let $\wt{\phi}_1, \dots, \wt{\phi}_t$ denote the rows of $\wt{\Phi}_t$. It is not hard to see that $\|\wt{\phi}_i\|_{\psi_2} \leq K$, for any $i \in [t]$. Further, for any $i \in [t]$, we have 
$$
\left\|\E\left[\wt{\phi}_i\wt{\phi}_i^T\right]\right\|_{op} \leq \left\|\E\left[\phi_i\phi_i^T\right]\right\|_{op} \leq \gamma.
$$
Thus, applying the triangle inequality, Lemma~\ref{lem:ext:noise_bound}, and Lemma~\ref{lem:ext:noise_cov}, we have, with probability at least $1 - \delta$
\begin{align*}
\left\|\wt{\Phi}_t\right\|_{op}^2 &= \left\|\wt{\Phi}_t^T\wt{\Phi}_t\right\|_{op} \\
&\leq \left\|\wt{\Phi}_t^T\wt{\Phi}_t - \E\left[\wt{\Phi}_t^T\wt{\Phi}_t\right]\right\|_{op} + \left\|\E\left[\wt{\Phi}_t^T\wt{\Phi}_t\right]\right\|_{op} \\
&\leq  K^2C_2\left(\sqrt{r} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)\left\{\sqrt{t} + \sqrt{r} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right\} + t\gamma.
\end{align*}
Taking square roots yields the desired result.

\end{proof}

\begin{lemma}
\label{lem:int:mixture}
Let $W \subset \R^d$ be a fixed subspace with $\dim(W) = r$. Let $a \in [A]$ and $\delta \in (0, 1)$ be arbitrary. Then, there is a universal constant $C > 0$ such that, with probability at least $1 - \delta$, simultaneously for all $t \geq 1$, we have 
\begin{align*}
\left\|\cV_t^W(a)^{-1/2}\vZ_t^W(a)^T\Xi_t(a)\right\|_2 &\leq CK\sqrt{2\log\left(\frac{1}{\delta}\sqrt{\det\left(\rho^{-1}\cV_t^W(a)\right)}\right)}\\
&\leq CK\sqrt{2\left[\frac{r}{2}\log\left(1 + \frac{\sigma_1^2(\cV_t^W(a))}{\rho}\right) + \log\left(\frac{1}{\delta}\right)\right]} \\
&\leq CK\sqrt{2\left[\frac{r}{2}\log\left(1 + \frac{\sigma_1^2(\cV_t(a))}{\rho}\right) + \log\left(\frac{1}{\delta}\right)\right]}
\end{align*}

\end{lemma}

\begin{proof}
Let $N_a := \left\{s \geq 1 : a_t = a\right\}$ be the set of rounds on which action $a \in [A]$ was selected, and let $N_a(t) := N_a \cap [t]$. Define the filtration $(\calF_t)_{t \in N_a}$ by $\calF_{t} := \sigma(Z_s : s \in N_a(t)) \bigwedge \sigma(\epsilon_s : s \in N_a(t - 1))$. Observe that the process $(S_t)_{t \in N_a}$ defined by
$$
S_t := \vZ^W_t(a)^T\Xi_t(a) = \sum_{s \in N_a(t)}\xi_s Z_s\vP^W_s
$$
is a martingale with respect to $(\calF_t)_{t \in N_a}$ taking values in $W \subset \R^d$, and that, by assumption, $\xi_t$ is $\sigma$-subGaussian conditioned on $\calF_{s}$, where $s \in N_a(t)$ is the largest value satisfying $s < t$. Consequently, since $\cV_t^W(a) = \sum_{s \in N_a(t)} (Z_s\vP^W_s)(Z_s \vP_s^W)^T + \rho I_d$, by Lemma~\ref{lem:ext:mixture}, we have, with probability at least $1 - \delta$
\begin{align*}
\left\|\cV_t^W(a)^{-1/2}\vZ^W_t(a)^T\Xi_t(a)\right\|_2 &= \left\|\cV_t^W(a)^{-1/2}S_t\right\|_2 \\
&\leq \sqrt{2\log\left(\frac{1}{\delta}\sqrt{\det\left(\rho^{-1}\cV^W_t(a)\right)}\right)},
\end{align*}
which proves the first inequality.

The second inequalilty now follows immediately from Lemma~\ref{lem:ext:det_trace}. More specifically, we know $\sum_{s \in N_a(t)}(Z_s\vP^W_s)(Z_s \vP_s^W)^T = \vZ_t^W(a)^T\vZ_t^W(a)$ is a matrix of rank at most $r$, and thus
$$
\log\det\left(\rho^{-1}\cV_t^W(a)\right) \leq r\log\left(1 + \frac{\sigma_1(\cV_t^W(a))}{\rho}\right).
$$
Plugging this into the right hand side of the first inequality yields the second inequality.
\end{proof}

\begin{lemma}
\label{lem:int:sv_conc}
Let $t \in [T]$ and $\delta \in (0, 1)$ be arbitrary. Then, there are universal constants $C_1, C_2 > 0$ such that, with probability at least $1 - \delta$, we have, simultaneously for all $i \in [r]$,
\begin{align*}
\left|\sigma_i(\vZ_t) - \sigma_i(\vX_t)\right| &\leq C_1\sigma\sqrt{\left(\sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)\left\{\sqrt{t} + \sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right\} + t\gamma} \\
&\leq C_2\sigma(\gamma \lor 1)\left(\sqrt{d} + \sqrt{t} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)
\end{align*}

In particular, if $\frac{\sigma_r(\vX_t)}{\sigma\left(\sqrt{t} + \sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)} \geq 2C_2$, we have, with probability at least $1 - \delta$,
$$
\sigma_r(\vZ_t) \geq \frac{\sigma_r(\vX_t)}{2},
$$

\end{lemma}

\begin{proof}
    By Lemma~\ref{lem:ext:weyl}, we know, for any $i \in [r]$, we have 
    $$
    \left|\sigma_i(\vZ_t) - \sigma_i(\vX_t)\right| \leq \left\|\vZ_t - \vX_t\right\|_{op} = \left\|\Epsilon_t\right\|_{op}.
    $$
    Next, letting $W = \R^d$ in Lemma~\ref{lem:int:cov_noise}, we see that there are constants $C_1, C_2 > 0$ such that, with probability at least $1 - \delta$, we have
    \begin{align*}
    \|\Epsilon_t\|_{op} &\leq C_1\sigma\sqrt{\left(\sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)\left\{\sqrt{t} + \sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right\} + t\gamma} \\
    &\leq C_2\sigma(\gamma \lor 1)\left(\sqrt{d} + \sqrt{t} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right),
    \end{align*}
    which proves the first inequality. Now, suppose $\frac{\sigma_r(\vX_t)}{\sigma\left(\sqrt{d} + \sqrt{t} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)} \geq  2C_2$. Then, we have, with probability at least $1 - \delta$,
    \begin{align*}
    \sigma_i(\vZ_t) &\geq \sigma_i(\vX_t) - C_2\sigma\left(\sqrt{t} + \sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right) \\
    &= \sigma_i(\vX_t) - \sigma_i(\vX_t)\frac{C_2\sigma\left(\sqrt{t} + \sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)}{\sigma_i(\vX_t)} \\
    &\geq \frac{\sigma_i(\vX_t)}{2},
    \end{align*}
    which proves the second result.

\end{proof}

\begin{lemma}
\label{lem:int:op_conc}
Let $\delta \in (0, 1)$, $a \in [A]$, and $t \in [T]$ be arbitrary. Then, there are universal constants $C_1, C_2 > 0$ such that, with probability at least $1 - \delta$, simultaneously for all subspaces $W \subset \R^d$, we have 
\begin{align*}
&\sigma_1(\vZ_t^W(a)^T\vZ_t^W(a)) \leq 2\sigma_1(\vX_t(a)^T\vX_t(a)) + 2\sigma_1(\Epsilon_t(a)^T\Epsilon_t(a)) \\
&\leq 2\sigma_1(\vX_t(a)^T\vX_t(a)) + 2C_1\sigma^2\left[\left(\sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)\left\{\sqrt{t} + \sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right\} + t\gamma\right] \\
&\leq 2\sigma_1(\vX_t(a)^T\vX_t(a)) + 2C_2\sigma^2(\gamma\lor1)\left(\sqrt{d} + \sqrt{t} + \log\left(\frac{1}{\delta}\right)\right)^2
\end{align*}
\end{lemma}

\begin{proof}
    First, observe that, for any subspace $W \subset \R^d$,
    \begin{align*}
        \sigma_1(\vZ_t(a)^T\vZ_t(a)) &= \sup_{x \in \R^d :\|x\| = 1}x^T\vZ_t(a)^T\vZ_t(a)x \\
        &\geq \sup_{x \in W : \|x\| = 1}x^T\vZ_t(a)^T\vZ_t(a)x \\
        &= \sup_{x \in W : \|x\| = 1} x\vP^W\vZ_t(a)^T\vZ_t(a)\vP^Wx \\
        &= \sup_{x \in W : \|x\| = 1} x\vZ_t^W(a)^T\vZ_t^W(a)x \\
        &=\sigma_1(\vZ_t^W(a)^T\vZ_t^W(a)).
    \end{align*}
    Next observe 
    $$
    \mathbf{0} \preceq (\vX_t(a) - \Epsilon_t(a))^T(\vX_t(a) - \Epsilon_t(a)) = \vX_t(a)^T\vX_t(a) - \vX_t(a)^T\Epsilon_t(a) - \Epsilon_t(a)^T\vX_t(a) + \Epsilon_t(a)^T\Epsilon_t(a).
    $$
    Rearranging the above yields 
    $$
    \vX_t(a)^T\Epsilon_t(a) + \Epsilon_t(a)^T\vX_t(a) \preceq \vX_t(a)^T\vX_t(a) + \Epsilon_t(a)^T\Epsilon_t(a).
    $$
    Leveraging this information, we have that
    \begin{align*}
    \vZ_t(a)^T\vZ_t(a) &= (\vX_t(a) + \Epsilon_t(a))^T(\vX_t(a) + \Epsilon_t(a)) \\
    &= \vX_t(a)^T\vX_t(a) + \vX_t(a)^T\Epsilon_t(a) + \Epsilon_t(a)^T\vX_t(a) + \Epsilon_t(a)^T\Epsilon_t(a) \\
    &\preceq 2\vX_t(a)^T\vX_t(a) + 2\Epsilon_t(a)^T\Epsilon_t(a).
    \end{align*}
    This implies the (deterministic) bound
    $$
    \sigma_1(\vZ_t^W(a)^T\vZ_t^W(a)) \leq 2\sigma_1(\vX_t(a)^T\vX_t(a)) + 2\sigma_1(\Epsilon_t(a)^T\Epsilon_t(a)).
    $$
    Now, by Lemma~\ref{lem:int:cov_noise}, we have that, with probability at least $1 - \delta$,
    \begin{align*}
    \sigma_1(\Epsilon_t(a)^T\Epsilon_t(a)) &\leq C_1^2\sigma^2\left[\left(\sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)\left\{\sqrt{t} + \sqrt{d} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right\} + t\gamma\right] \\
    &\leq C_2\sigma^2(\gamma\lor1)\left(\sqrt{d} + \sqrt{t} + \sqrt{\log\left(\frac{1}{\delta}\right)}\right)^2
    \end{align*}
    for some universal constants $C_1, C_2 > 0$. Combining this line with the previous yields the desired, high probability result.
    
\end{proof}

==> arxiv/regret.tex <==
\section{Regret analysis}
%
Let $a_i^* := \arg\max_{a \in [A]} \langle \theta(a), Z_i \rangle$. 
%
\begin{equation*}
\begin{aligned}
    R(n) &:= \sum_{i=1}^n \langle \theta(a_i^*) - \theta(a_i), X_i \rangle\\
    %
    &= \sum_{i=1}^n \underbrace{\langle \theta(a_i^*) - \theta(a_i), Z_i \rangle}_{T_1} + \underbrace{\langle \theta(a_i) - \theta(a_i^*), \epsilon_i \rangle}_{T_2}
\end{aligned}
\end{equation*}
%
Assume that $\langle \theta(a_i^*) - \theta(a_i), X_i \rangle \leq 2$. 
%
Focusing on $T_2$, we see that 
%
\begin{equation*}
\begin{aligned}
    \langle \theta(a_i) - \theta(a_i^*), \epsilon_i \rangle &\leq \max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle\\
    %
    &= \max_{a,a' \in [A]} \langle B(\theta(a) - \theta(a')), B\epsilon_i \rangle\\
    %
    &= \max_{a,a' \in [A]} \langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle\\
\end{aligned}
\end{equation*}
%
where $B \in \mathbb{R}^{d \times d}$ is the orthonormal matrix such that the first $r$ columns span $W$ and $[x]_r$ denotes the top $r$ elements of the vector $x$. 
%
Note that $\langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle$ is $2L \sigma \sqrt{r}$-subgaussian.
%
\begin{equation*}
\begin{aligned}
    \mathbb{P}(\max_{a,a' \in [A]} \langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle > t ) &= \mathbb{P}( \cup_{a,a \in [A]} \langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle > t )\\
    %
    &\leq \sum_{a=1, a'=1}^A \mathbb{P}(\langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle > t )\\
    %
    &\leq A^2 \exp(\frac{-t^2}{4L^2r\sigma^2})
\end{aligned}
\end{equation*}
%
Inverting the bound, we get that 
%
\begin{equation*}
    \langle \theta(a_i) - \theta(a_i^*), \epsilon_i \rangle \leq 2L\sigma \sqrt{2r\log(A/\delta)}
\end{equation*}
%
with probability $1 - \delta$. 
%

Returning to $T_1$, observe that with high probability,
%
\begin{equation*}
    \langle \theta(a_i^*), Z_i \rangle \leq \text{UCB}(a_i^*) \leq \text{UCB}(a_i) = \langle \Tilde{\theta}(a_i), Z_i \rangle
\end{equation*}
%
and so
%
\begin{equation*}
\begin{aligned}
    \langle \theta(a_i^*) - \theta(a_i), Z_i \rangle &\leq \langle \Tilde{\theta}(a_i) - \theta(a_i), Z_i \rangle\\
    %
    &\leq \| \Tilde{\theta}(a_i) - \theta(a_i) \|_{V_{i-1}(a_i)} \|Z_i\|_{V_{i-1}^{-1}(a_i)}\\
    %
    &\leq 2\sqrt{\beta_{i-1}(a_i)}\|Z_i\|_{V_{i-1}^{-1}(a_i)}\\
\end{aligned}
\end{equation*}
%
Putting $T_1$ and $T_2$ together along with the boundedness assumption, we can bound instantaneous regret by 
\begin{equation*}
    2 \wedge (2\sqrt{\beta_{i-1}(a_i)}\|Z_i\|_{V_{i-1}^{-1}(a_i)} + 2L\sigma \sqrt{2r\log(A/\delta)}) \leq 2(1 \wedge \sqrt{\beta_{i-1}(a_i)}\|Z_i\|_{V_{i-1}^{-1}(a_i)}) + 2L\sigma \sqrt{2r\log(A/\delta)}
\end{equation*}
%
Therefore we can bound regret as
%
\begin{equation}
\begin{aligned}
    R(n) &\leq \sum_{i=1}^n 2(1 \wedge \sqrt{\beta_{i-1}(a_i)}\|Z_i\|_{V_{i-1}^{-1}(a_i)}) + \sum_{i=1}^n 2L\sigma \sqrt{2r\log(A/\delta)}\\
    %
    &\leq 2\sqrt{n \sum_{i=1}^n (1 \wedge \sqrt{\beta_{i-1}(a_i)}\|Z_i\|_{V_{i-1}^{-1}(a_i)})^2} + 2Ln\sigma \sqrt{2r\log(An/\delta)}\\
    %
    &\leq 2 \sqrt{n \beta_n \sum_{i=1}^n (1 \wedge \|Z_i\|^2_{V_{i-1}^{-1}(a_i)})} + 2Ln\sigma \sqrt{2r\log(An/\delta)}\\
\end{aligned}
\end{equation}
%
where we assume that $\beta_n = \max_{a \in [A]} \beta_n(a) \geq 1$

\iffalse
\begin{equation*}
\begin{aligned}
    \sum_{i=1}^n \langle \theta(a_i) - \theta(a_i^*), \epsilon_i \rangle &\leq \sum_{i=1}^n \max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle\\
    %
    &= \underbrace{\sum_{i=1}^n (\max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle - \mathbb{E} \max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle)}_{T_1} + \sum_{i=1}^n \underbrace{\mathbb{E} \max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle}_{T_2}\\
    %
\end{aligned}
\end{equation*}
%
We bound each term separately, starting with $T_2$.
%
\begin{equation*}
\begin{aligned}
    \mathbb{E} \max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle &= \mathbb{E} \max_{a,a' \in [A]} \langle B(\theta(a) - \theta(a')), B\epsilon_i \rangle\\
    %
    &= \mathbb{E} \max_{a,a' \in [A]} \langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle\\
    %
    &= \frac{1}{s} \mathbb{E} \log \exp s \max_{a,a' \in [A]} \langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle\\
    %
    &\leq \frac{1}{s} \log \mathbb{E} \exp s \max_{a,a' \in [A]} \langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle\\
    %
    &= \frac{1}{s} \log \mathbb{E} \max_{a,a' \in [A]} \exp s \langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle\\
    %
    &\leq \frac{1}{s} \log \sum_{a=1, a'=1}^A \mathbb{E} \exp s \langle [B(\theta(a) - \theta(a'))]_r, [B\epsilon_i]_r \rangle\\
    %
    &= \frac{1}{s} \log \sum_{a=1, a'=1}^A \Pi_{j=1}^r \mathbb{E} \exp s [B(\theta(a) - \theta(a'))]_r [j], [B\epsilon_i]_r [j]\\
    %
    &\leq \frac{1}{s} \log \sum_{a=1, a'=1}^A \Pi_{j=1}^r \exp \frac{1}{2} s^2 \sigma^2 ([B(\theta(a) - \theta(a'))]_r [j])^2\\
    %
    &\leq \frac{1}{s} \log \sum_{a=1, a'=1}^A \exp s^2 \sigma^2 L^2\\
    %
    &= \frac{1}{s} \log A^2 \exp s^2 \sigma^2 L^2\\
    %
    &= \frac{2 \log A}{s} + s \sigma^2 L^2
\end{aligned}
\end{equation*}
%
where $s \in \mathbb{R}$ is arbitrary, $B \in \mathbb{R}^{d \times d}$ is the orthonormal basis such that $W$ is spanned by the first $r$ coordinates, $[x]_r$ denotes the truncation of vector $x$ to the top $r$ coordinates, and the third inequality follows from the rotational invariance of the Gaussian distribution. 
%
Picking $s$ to balance the two terms, we get that $\mathbb{E} \max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle \leq 2 \sigma L \sqrt{2 \log A}$. 
%
\fi 
\iffalse
We now turn our attention to $T_1$. Note that 
%
\begin{equation*}
\begin{aligned}
    &\mathbb{P}(\sum_{i=1}^n \left(\max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle - \mathbb{E} \max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle \right) \geq t)\\ 
    %
    = &\mathbb{P}(\sum_{i=1}^n \left(\cup_{a,a' \in [A]} (\langle \theta(a) - \theta(a'), \epsilon_i \rangle - \mathbb{E} \langle \theta(a) - \theta(a'), \epsilon_i \rangle \right) \geq t) )\\
    %
    \leq &\sum_{a=1, a'=1}^{A} \mathbb{P}(\langle \theta(a) - \theta(a'), \epsilon_i \rangle - \mathbb{E} \langle \theta(a) - \theta(a'), \epsilon_i \rangle \geq t)
\end{aligned}
\end{equation*}
\fi 







\iffalse
\begin{equation*}
\begin{aligned}
    \sum_{i=1}^n \langle \theta(a_i) - \theta(a_i^*), \epsilon_i \rangle &\leq \sum_{i=1}^n \max_{a,a' \in [A]} \langle \theta(a) - \theta(a'), \epsilon_i \rangle\\
    %
    &\leq \sum_{i=1}^n 2 \sigma L \sqrt{d} \sqrt{2\log(nA^2/\delta)}\\
    %
    &\leq 4 \sigma n L \sqrt{d \log(nA/\delta)}
\end{aligned}
\end{equation*}
%
with probability at least $1 - \delta$, where the second inequality follows from the fact that $\langle \theta(a_i^*) - \theta(a), \epsilon_i \rangle$ is a $2 \sigma L \sqrt{d}$-subGaussian random variable, the maximal inequality for subGaussian random variables, and a union bound. 
%
Note that $\frac{1}{nd} \cdot 4 \sigma n L \sqrt{d \log(nA/\delta)} \rightarrow 0$ as $n, d \rightarrow \infty$ if $r \log n \leq d$.
%
\fi 
%

